Unraveling Cross-Modality Knowledge Conflicts in Large Vision-Language Models

Large Vision-Language Models (LVLMs) have demonstrated impressive capabilities for capturing and reasoning over multimodal inputs. However, these models are prone to parametric knowledge conflicts, which arise from inconsistencies of represented knowledge between their vision and language components. In this paper, we formally define the problem of $\textbf{cross-modality parametric knowledge conflict}$ and present a systematic approach to detect, interpret, and mitigate them. We introduce a pipeline that identifies conflicts between visual and textual answers, showing a persistently high conflict rate across modalities in recent LVLMs regardless of the model size. We further investigate how these conflicts interfere with the inference process and propose a contrastive metric to discern the conflicting samples from the others. Building on these insights, we develop a novel dynamic contrastive decoding method that removes undesirable logits inferred from the less confident modality components based on answer confidence. For models that do not provide logits, we also introduce two prompt-based strategies to mitigate the conflicts. Our methods achieve promising improvements in accuracy on both the ViQuAE and InfoSeek datasets. Specifically, using LLaVA-34B, our proposed dynamic contrastive decoding improves an average accuracy of 2.24%.

==> table/cd_metric.tex <==
\begin{tabular}{lll}
    \toprule
    \textbf{Models} & \textbf{ViQuAE} & \textbf{InfoSeek} \\
    \midrule
    LLaVA-7b                & 1.7326                              & 0.7944                                \\
    LLaVA-13b               & -0.2137                             & -0.3225                               \\
    LLaVA-34b               & -0.2971                             & 0.4141                                \\
    \bottomrule
\end{tabular}


==> table/cd_metric_samplewise.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{lcccccc}
    \toprule
    \multirow{2}{*}{\textbf{Models}} & \multicolumn{3}{c}{\textbf{ViQuAE}} & \multicolumn{3}{c}{\textbf{InfoSeek}} \\
    \cline{2-7}
     & \textbf{Avg.} & \textbf{w/o conflict} & \textbf{w. conflict} & \textbf{Avg.} & \textbf{w/o conflict} & \textbf{w. conflict} \\
    \hline
    LLaVA-7b & 2.92 & 2.88 & 2.95 & 1.89 & 1.95 & 1.83 \\
    LLaVA-13b & 1.21 & 0.66 & 2.85 & 1.14 & 0.77 & 1.47 \\
    LLaVA-34b & 0.94 & 0.59 & 1.65 & 1.46 & 1.42 & 1.53 \\
    \bottomrule
\end{tabular}


==> table/cd_results.tex <==
\begin{tabular}{l|ccc|ccc}
    \toprule
    \multirow{2}{*}{Model} & \multicolumn{3}{c|}{ViQuAE} & \multicolumn{3}{c}{InfoSeek} \\ \cline{2-7} 
                           & Acc$\uparrow$     & CR$\downarrow$      & CR-$\Delta$Acc$\downarrow$  & Acc$\uparrow$     & CR$\downarrow$     & CR-Acc$\downarrow$    \\ \hline
    LLaVA-7b               & 44.29   & 58.52   & 22.49   &         &        &           \\
    LLaVA-13b              & 22.86   & 83.42   & 40.84   &         &        &           \\
    LLaVA-34b              & 29.53   & 78.47   & 27.01   &         &        &           \\
    InstructBlip           &         &         &         &         &        &           \\
    \bottomrule
\end{tabular}

